Cross-Instance Gaussian Splatting Registration via Geometry-Aware Feature-Guided Alignment

We present Gaussian Splatting Alignment (GSA), a novel method for aligning two independent 3D Gaussian Splatting (3DGS) models via a similarity transformation (rotation, translation, and scale), even when they are of different objects in the same category (e.g., different cars). In contrast, existing methods can only align 3DGS models of the same object (e.g., the same car) and often must be given true scale as input, while we estimate it successfully. GSA leverages viewpoint-guided spherical map features to obtain robust correspondences and introduces a two-step optimization framework that aligns 3DGS models while keeping them fixed. First, we apply an iterative feature-guided absolute orientation solver as our coarse registration, which is robust to poor initialization (e.g., 180 degrees misalignment or a 10x scale gap). Next, we use a fine registration step that enforces multi-view feature consistency, inspired by inverse radiance-field formulations. The first step already achieves state-of-the-art performance, and the second further improves results. In the same-object case, GSA outperforms prior works, often by a large margin, even when the other methods are given the true scale. In the harder case of different objects in the same category, GSA vastly surpasses them, providing the first effective solution for category-level 3DGS registration and unlocking new applications. Project webpage: https://bgu-cs-vil.github.io/GSA-project/

==> macros.tex <==
 %--------------------------------------------
% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
% \def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} 
% \def\wrt{with respect to }  % The extra space at the end means \wrt blah would 
% not end up as ``with respect toblah''. 
 
\def\dof{d.o.f\onedot}
% \def\etal{\emph{et al}\onedot}
\def\etal{\emph{et al}\onedot}
% \def\etal{\emph{et al}\onedot}
%
\def\iid{\emph{i.i.d}\onedot}
% \def\pdf{\emph{p.d.f}\onedot}



\makeatother
%--------------------------------------------------

\newcommand{\FIG}{Fig.~}
\newcommand{\FIGS}{Figs.~}
\newcommand{\EQN}{Eq.~}
% \newcommand{\EQN}{Equation }
\newcommand{\EQNS}{Eqs.~}
% \newcommand{\EQNS}{Equations }

%\newcommand{\SEC}{Sec.~}.  Use \autoref or ~\autoref instead.



% integers
\newcommand{\ZZ}{\ensuremath{\mathbb{Z}}}
\newcommand{\RR}{\ensuremath{\mathbb{R}}}
\newcommand{\Rtwo}{\ensuremath{\RR^2}}
\newcommand{\Rthree}{\ensuremath{\RR^3}}
\newcommand{\Rfive}{\ensuremath{\RR^5}}

\newcommand{\Rsix}{\ensuremath{\RR^6}}

\newcommand{\Rn}{\ensuremath{\RR^n}}
\newcommand{\Rd}{\ensuremath{\RR^d}}
\newcommand{\Rk}{\ensuremath{\RR^k}}

% 
%positive integers
\newcommand{\Zplus}{\ensuremath{\ZZ^+}}
%positive reals
\newcommand{\Rplus}{\ensuremath{\RR^+}}


% set notation
% \newcommand{\set}[1]{\ensuremath{{\left\{#1\right\}}}}
\newcommand{\set}[1]{\ensuremath{{\{#1\}}}}
\newcommand{\tuple}[1]{\ensuremath{{(#1)}}}
\newcommand{\tupleLarge}[1]{\ensuremath{{\left(#1\right)}}}
\newcommand{\argmin}[1]{\ensuremath{\operatorname*{arg\,min}_{#1}}}
\newcommand{\argmax}[1]{\ensuremath{\operatorname*{arg\,max}_{#1}}}



\newcommand{\InnerProduct}[2]{\left\langle #1,#2 \right\rangle}

\newcommand{\norm}[1]{{{\left\|#1\right\|}}}
\newcommand{\sign}[1]{{\mathrm{sign}\left(#1\right)}}

\newcommand{\ellTwo}{\ell_2}
\newcommand{\ellTwoNorm}[1]{\norm{#1}_{\ellTwo}}
\newcommand{\ellOne}{\ell_1}




\newcommand{\MATRIX}[2][cccccccccccccccccccc]{\left[
 \begin{array}{#1}
 #2
 \end{array}
\right]}

\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}



% homogeneous coordinates
\newcommand{\bxh}{\widetilde{\bx}}

\newcommand{\RED}[1]{{{\color{red}{#1}}}}  
\newcommand{\BLUE}[1]{{{\color{blue}{#1}}}}
\newcommand{\GREEN}[1]{{{\color{green}{#1}}}}
\newcommand{\MAGENTA}[1]{{{\color{magenta}{#1}}}}  



\newcommand{\FREIFELD}[1]{\textbf{\MAGENTA{[FREIFELD says: #1]}}}
% Make your own

\newcommand{\AMOYAL}[1]{\textbf{\BLUE{[Roy says: #1]}}}

\newcommand{\TBD}{\RED{[TBD]}}
%\newcommand{\TODO}[1]{\RED{[TODO: #1]}}




% In python: print_iterable(['\\bmdefine\\b{0}'.format(x)+'{'+x+'}' for x in 
% string.ascii_letters])

\bmdefine\ba{a}
\bmdefine\bb{b}
\bmdefine\bc{c}
\bmdefine\bd{d}
\bmdefine\be{e}
% \bmdefine\bf{f}  # Clashes with a standard command
\bmdefine\boldf{f}
\bmdefine\bg{g}
\bmdefine\bh{h}
\bmdefine\bi{i}
\bmdefine\bj{j}
\bmdefine\bk{k}
\bmdefine\bl{l}
\bmdefine\bm{m}
\bmdefine\bn{n}
\bmdefine\bo{o}
\bmdefine\bp{p}
\bmdefine\bq{q}
\bmdefine\br{r}
\bmdefine\bs{s}
\bmdefine\bt{t}
\bmdefine\bu{u}
\bmdefine\bv{v}
\bmdefine\bw{w}
\bmdefine\bx{x}
\bmdefine\by{y}
\bmdefine\bz{z}
\bmdefine\bA{A}
\bmdefine\bB{B}
\bmdefine\bC{C}
\bmdefine\bD{D}
\bmdefine\bE{E}
\bmdefine\bF{F}
\bmdefine\bG{G}
\bmdefine\bH{H}
\bmdefine\bI{I}
\bmdefine\bJ{J}
\bmdefine\bK{K}
\bmdefine\bL{L}
\bmdefine\bM{M}
\bmdefine\bN{N}
\bmdefine\bO{O}
\bmdefine\bP{P}
\bmdefine\bQ{Q}
\bmdefine\bR{R}
\bmdefine\bS{S}
\bmdefine\bT{T}
\bmdefine\bU{U}
\bmdefine\bV{V}
\bmdefine\bW{W}
\bmdefine\bX{X}
\bmdefine\bY{Y}
\bmdefine\bZ{Z}


\bmdefine\balpha{\alpha}
\bmdefine\bbeta{\beta}
\bmdefine\bgamma{\gamma}

\bmdefine\bdelta{\delta}
\bmdefine\btheta{\theta}
\bmdefine\blambda{\lambda}
\bmdefine\bphi{\phi}
\bmdefine\bxi{\xi}
\bmdefine\bzeta{\zeta}
\bmdefine\boldeta{\eta}
\bmdefine\bpi{\pi}

\bmdefine\bmu{\mu}
\bmdefine\brho{\rho}
\bmdefine\bomega{\omega}
\bmdefine\bOmega{\Omega}
\bmdefine\bPi{\Pi}

\bmdefine\bvarepsilon{\varepsilon}

\bmdefine\bDelta{\Delta}

\bmdefine\bTheta{\Theta}

\bmdefine\bSigma{\Sigma}
\bmdefine\bPsi{\Psi}
\bmdefine\bLambda{\Lambda}



\bmdefine\bzero{0}
\bmdefine\bone{1}
\bmdefine\binfty{\infty}

 \newcommand{\indicator}{\mathbbm{1}}



==> preamble_old.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\usepackage{bm}
\usepackage{capt-of} % in preamble


\usepackage[linesnumbered,algoruled,noend,noline]{algorithm2e}

% SPACES
\usepackage{booktabs, array, tabularx} % if not already loaded


% In python 
% print_iterable(['\\newcommand{\\'+'{0}cal'.format(x)+'}{\\mathcal{'+x+'}}' 
% for x in string.ascii_uppercase])
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}
\defcitealias{Oquab:arXiv:2023:DINOv2}{DINOv2}
\defcitealias{Zhang:CVPR:2024:TellingLeftRight}{TellingLeftRight}
\defcitealias{Mariotti:CVPR:2024:ViewpointSphereMap}{SphereMap}





%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> sec/1_intro_OLD.tex <==
\RED{
\section{Introduction -OLD} \label{Sec:Intro}

The problem of 3D registration has been extensively studied in computer vision, particularly in 3D reconstruction and object alignment. Traditional registration methods, such as point cloud alignment using geometric descriptors, have made significant progress. However, the emergence of novel view synthesis (NVS) techniques, particularly Neural Radiance Fields (NeRF) and 3D Gaussian Splatting (3DGS), introduces new challenges in aligning and registering objects across different scenes, coordinate systems, and scales. 

The \textbf{scale and coordinate system variation} issue arises due to the inherent nature of \textit{Structure-from-Motion} (SfM) in image-based 3D reconstruction. Since SfM estimates a scene’s structure solely from monocular images, the lack of absolute depth information leads to arbitrary scale assignment, causing inconsistencies in scale across different reconstructions. Additionally, variations in the input images influence the choice of the coordinate system, as SfM optimizes camera poses based on the available viewpoints. As a result, reconstructions from different scenes may have not only inconsistent scales but also misaligned coordinate frames, making direct alignment challenging without additional transformations.

While NeRF registration is inherently challenging due to its implicit scene representation, recent efforts such as DReg-NeRF have attempted to extract explicit features for alignment. However, 3D Gaussian Splatting (3DGS) offers an explicit representation, making it a more suitable candidate for object-level registration. Despite its advantages in efficient rendering and direct manipulation, 3DGS registration remains an underexplored problem, particularly in handling scale variations and structural differences between different instances of the same object.

Existing approaches for 3DGS registration have primarily focused on scene-level alignment. GaussReg, for example, introduced a coarse-to-fine pipeline that leverages Iterative Closest Point (ICP) \cite{Besl:SensorFusion:1992:ICP} for alignment and image-guided refinement for fine registration. While GaussReg achieves fast and accurate registration, it is designed primarily for scene-level alignment and does not explicitly tackle object-level registration and different scale variations. Moreover, its reliance on geometric correspondences limits its ability to handle significant shape variations, making it less effective for aligning structurally different objects within the same category.

Unlike prior methods that rely on semantic feature extractors (\eg, DINO) but lack geometric awareness, we use the viewpoint-guided spherical features from Mariotti~\cite{Mariotti:CVPR:2024:ViewpointSphereMap}~\etal , which are explicitly designed to handle spatial ambiguity. These features were designed to distinguish between left-right and view-dependent transformations, improving the robustness of our category-level registration.


In this paper, we propose a novel approach that addresses these limitations by introducing \textbf{feature-enhanced Gaussian Splatting registration}. Specifically, we incorporate learned \textit{3D geometry-aware semantic features} into the explicit Gaussian splats, enabling more robust correspondences across different instances. This results in higher registration accuracy, improved robustness to scale variations, and better handling of structural differences between models. As illustrated in \autoref{Fig:Method}, our method enables object-wise replacement and synchronized novel view synthesis across multiple object instances while maintaining geometric consistency. Furthermore, to the best of our knowledge, our work is the first to offer a solution for \textbf{category-level registration} in the NVS domain.

\subsection{Key Contributions}
\begin{itemize}
    \item \textbf{Feature-Enhanced Gaussian Splatting Registration:} We introduce a new 3D registration method that augments the Gaussian Splatting representation with learned geometric-semantic features, enabling robust alignment across different object instances, including those with scale variations and structural differences.
    
    \item \textbf{Accurate Object-Level Registration:} Our method achieves state-of-the-art registration accuracy, significantly outperforming previous 3DGS registration methods, including GaussReg, in handling variations in scale and viewing conditions between different reconstructions of the same object. 
    
    \item \textbf{First Category-Level Registration Solution in NVS:} To the best of our knowledge, we are the first to offer a category-level registration approach within the NVS domain, extending Gaussian Splatting registration beyond individual objects to structurally varying instances within the same category.
    
    \item \textbf{Novel View Synthesis Applications:} We demonstrate that accurate object-level registration enables new applications, such as synchronized multi-object novel view synthesis and multi-view consistent object replacement in 3D scenes. These capabilities highlight the practical benefits of our method for scene manipulation and reconstruction.
\end{itemize}

Through extensive experiments, we show that our approach outperforms existing methods in terms of registration accuracy and robustness. Our results suggest that this method can serve as a strong foundation for future research in registration-based novel view synthesis, enabling more flexible and accurate 3D object alignment.



==> sec/3_method_OLD.tex <==
\section{Method}
\FREIFELD{We need to rewrtie this paragraph}
We consider two 3D Gaussian Splatting models representing objects from the same category, sharing similar geometric-semantic characteristics. For each model, we assume the availability of \( N \) and \( M \) images, respectively, along with their corresponding camera poses. The images can be obtained through image rendering by systematically rotating and translating the camera around the object or directly using the available training images. If the 3D model is unavailable and only the training images are available, the camera poses can be reconstructed using established Structure-from-Motion (SfM) algorithms such as COLMAP~\cite{Schoenberger:CVPR:2016:sfm}, which is the current practice.


\subsection{3D Gaussian Splatting with Enhanced Features}

Using an off-the-shelf segmentation model (\eg, SAM \cite{Kirillov:ICCV:2023:SAM}), we first apply an image segmentation process to isolate the object of interest from each image, producing a masked version of the image that contains only the segmented object. Let the original image be denoted by \( I_k \), and the masked image (containing the object) be denoted by \( I_k^{\text{masked}} \). Additionally, we use a 3D geometry-aware feature extraction process to extract feature maps from the original image and the masked image, resulting in the feature map \( F_k \) for the original image and the masked feature map \( F_k^{\text{masked}} \) for the segmented object.

To obtain the masked image \( I_k^{\text{masked}} \), we apply a mask operation on the original image \( I_k \), isolating the object of interest. Similarly, the feature map \( F_k^{\text{masked}} \) is obtained by applying the mask on the feature map \( F_k \), which corresponds to the object of interest.

\begin{align}
I_k^{\text{masked}} &= \text{Mask}(I_k) \\
F_k^{\text{masked}} &= \text{FeatureExtractor}(I_k) \odot I_k^{\text{masked}}
\end{align}
where $\odot$ is the Hadamard product (\ie, element-wise product). 
Next, we train a 3D Gaussian Splatting model, either by fine-tuning an existing 3D object model or by training from scratch using images of the masked object, along with the corresponding masked feature maps.

These enhanced Gaussians form a 3D radiance field, where each Gaussian contains information about its 3D mean, covariance, opacity, color (represented, as is customary in 3DGS, using spherical harmonics), and a semantic geometry-aware feature vector.

Let the 3D coordinates of the mean of Gaussian $i$ be denoted by \( \bp_i = (x_i, y_i, z_i) \), its covariance matrix by \( \bSigma_i \), its opacity by \( \alpha_i \), and its spherical harmonics by \( SH_i \). The feature vector associated with the \( i \)-th Gaussian is denoted by \( \boldf_i \). Thus, each Gaussian is described by:

\begin{align}
\mathcal{N}(\bp_i, \bSigma_i, \balpha_i, \mathbf{SH}_i, \boldf_i)
\end{align}

During the training of the 3D Gaussian Splatting model, we optimize all Gaussian properties through a combined loss function that incorporates both photometric reconstruction and feature learning:

\begin{align}
\Lcal = \Lcal_{\mathrm{rgb}} + \lambda\Lcal_f
\end{align}

where \(\Lcal_{\mathrm{rgb}}\) is the photometric loss combining $\ell_1$ and 
Structural Similarity Index Measure (SSIM)~\cite{Wang2003MultiscaleSS}  losses:

\begin{align}
\Lcal_{\mathrm{rgb}} = (1 - \alpha)\Lcal_1(I, \hat{I}) + \alpha\Lcal_{\mathrm{SSIM}}(I, \hat{I})
\end{align}

\FREIFELD{Should probaly say something about $\alpha$. E.g., that it's a user-defined hyperparemter, in (0,1), and in our experiment it is set to XYZ}

and \(\Lcal_f\) is the feature loss computed as the $\ell_1$ distance between the rendered and target feature maps:

\begin{align}
\Lcal_f = \|F_r(I) - F_t(I)\|_{\ell_1}
\end{align}

The rendering process for both images and features follows the standard Gaussian splatting procedure. For each view, we compute the contributions of all Gaussians through:

\begin{align}
C = \sum_{i \in \Xcal} \bc_i\alpha_i, \quad F_r = \sum_{i \in \Xcal} \boldf_i\alpha_i
\end{align}

where \(\bc_i\) is the RGB color contribution (computed from spherical harmonics) of Gaussian $i$, \(\alpha_i\) is its opacity, and \(\boldf_i\) is its feature vector. Here, \(\Xcal\) represents the set of all of the Gaussians that project to the current pixel.

During the training process, all Gaussian properties, including the means \( \bp_i \), covariances \( \bSigma_i \), opacities \( \alpha_i \), spherical harmonics \( SH_i \), and feature vectors \( \boldf_i \), are optimized simultaneously. However, the gradients of the feature vectors do not influence the optimization of the other properties. This is because the feature maps obtained from the feature extractor are typically low-resolution, patch-based, and not pixel-accurate. Allowing the feature gradients to affect the geometric properties could degrade the spatial reconstruction quality. By keeping the feature vectors independent in the backward pass, we ensure that the geometric structure of the scene remains intact while still enabling feature learning in parallel.

The result of this training process is a 3D Gaussian model where the rendered feature maps derived from the 3D model have enhanced semantic geometric meaning. These rendered feature maps have higher resolution than the original feature maps extracted by the feature extractor, enriching the representation with more accurate spatial details. The enhanced feature maps contribute to refining the model's understanding of the object's geometry while also improving the fidelity of the feature maps used for further tasks such as alignment.

By utilizing this enhanced representation, we can leverage the 3D semantic features to perform more accurate and robust alignment between models, taking advantage of the combined spatial and semantic cues embedded in the Gaussians as seen in \autoref{fig:enhanced_features}.
\subsection{Coarse Registration: Iterative Feature-guided Absolute Orientation Solver}
We present an approach for aligning 3D Gaussian models by iteratively solving the \emph{absolute orientation problem} \cite{horn1987closedquaternion}. The method operates by using the means of 3D Gaussians as points and randomly selecting a subset for alignment. Following a similar structure \FREIFELD{we need to make the gap from ICP sound larger} to iterative closest point methods, our approach alternates between two main steps: (1) establishing correspondences using geometric-aware feature matching and (2) solving for the optimal similarity transformation utilizing Horn's closed solution using orthonormal matrices \cite{horn1988closed}. Let \(\Pcal = \{\bp_i\}_{i=1}^N\) and \(\Qcal = \{\bq_j\}_{j=1}^M\) denote the source and target point clouds respectively, with associated feature vectors \(\mathcal{F}_\Pcal = \{\boldf_i\}_{i=1}^N\) and \(\mathcal{F}_\Qcal = \{\boldf_j\}_{j=1}^M\).

It is important to note that this representation is inherently noisy, as each 3D Gaussian effectively captures the spatial distribution of multiple points in the actual geometry. However, our method compensates for this potential imprecision through two key factors:

1. The semantic feature vectors associated with each Gaussian provide strong guidance for correspondence matching, helping to identify correct pairs even when the spatial positions are not perfectly aligned.

2. The similarity transformation captures the inherent scale variations that typically arise when reconstructing 3D models from images, where each model may be produced at a different scale. Unlike traditional rigid ICP \cite{Besl:SensorFusion:1992:ICP} methods, our approach leverages strong feature-based correspondences that enable robust and accurate scale estimation during alignment.

Despite working with this relatively coarse because of the noisy point cloud representation, this first step in our feature-guided point clouds registration achieves results comparable to state-of-the-art methods novel view synthesis registration methods. (\textcolor{red}{Roy: "comparable" if GaussReg authors provide the evaluation code and it achieves the same results they reported, or our coarse method will be also "SOTA"}).  This demonstrates that the semantic information encoded in our enhanced Gaussians effectively compensates for the reduced geometric precision.

The similarity transformation \(\Tcal(s, \bR, \bt)\) maps a point \(\bp\) to:
\begin{align}
\Tcal(\bp) = s \bR \bp + \bt
\end{align}
where \(s \in \mathbb{R}^+\) is the scale factor, \(\bR \in SO(3)\) is the rotation matrix, and \(\bt \in \mathbb{R}^3\) is the translation vector.



% \begin{figure*}[t]
%     \centering
%     \begin{tikzpicture}
%         % Include the image
%         \node[anchor=south west,inner sep=0] (image) at (0,0) 
%         {\includegraphics[width=\textwidth]{./figures/method/slide1.jpg}};

%         % Overlaying text annotations
%         \begin{scope}[shift={(0,0)}, font=\bfseries]
%             \node at (10,8) {Train two independent};
%             \node at (10,7.5) {3DGS models};
%             \node at (10,7) {augmented by geometric};
%             \node at (10,6.5) {semantic features};

%             \node at (3,2) {3D means $u_i, u_j$ of $g_i \in \mathcal{G}_1,$};
%             \node at (3,1.5) {$g_i \in \mathcal{G}_2$ as point clouds};

%             \node at (6,1.2) {Coarse Registration};
%             \node at (6,0.8) {$T: (s, R, t)$};

%             \node at (12,1.2) {Fine Registration};
%             \node at (12,0.8) {$T^*: (s^*, R^*, t^*)$};

%             \node at (15,2) {Model $\mathcal{G}_2$ aligned};
%             \node at (15,1.5) {to model $\mathcal{G}_1$};

%             \node at (15,7.5) {Model $\mathcal{G}_1$ (color)};
%             \node at (15,6.5) {Model $\mathcal{G}_2$ (color)};

%             \node at (15,5) {Model $\mathcal{G}_1$ (features)};
%             \node at (15,4) {Model $\mathcal{G}_2$ (features)};
%         \end{scope}

%     \end{tikzpicture}
%     \caption{Annotated Image with TikZ}
%     \label{fig:annotated}
% \end{figure*}


% ------------- BACKUP ---------------
% \begin{figure*}
% \centering
% \begin{tikzpicture}[
% img/.style={rectangle, minimum width=3cm, minimum height=4cm},
% arrow/.style={->, >=latex, thick},
% every node/.style={font=\large}
% ]
% \node[font=\small] at (0.5,14) {(1)};
% \node[font=\small] at (0.5,10) {(2)};
% % First pair of images
% \node[img] (img1) at (4,14) {\includegraphics[width=6cm, height=3.0cm]{./figures/method/1_ver2.png}};
% \node[img] (img2) at (4,10) {\includegraphics[width=6cm, height=3.2cm]{./figures/method/2_ver2.png}};
% % Second image pair
% \node[img] (img3) at (12.7,14.5) {\includegraphics[width=6cm, height=4cm]{./figures/method/3_new.png}};
% \node[img] (img4) at (12.7,10.2) {\includegraphics[width=6cm, height=4cm]{./figures/method/4_new.png}};
% % Connection lines and arrow to first pair
% \draw[thick] (img1.east) -- (9,14);
% \draw[thick] (img2.east) -- (9,10);
% \draw[thick] (9,14) -- (9,11.5);
% \draw[thick] (9,10) -- (9,11.5);
% \draw[->, >=latex, thick, draw=black] (9,12) -- (10,12);
% % Arrow after image 3,4 with text
% \draw[->, >=latex, thick, draw=black] (15.5,12) -- (17,12);
% \node[font=\small, align=left] at (16.2,12.4) {3D Means as \\ Point Clouds};

% % Bottom row with SHORTER REGISTRATION ARROWS
% \node[img] (img5) at (2,5.5) {\includegraphics[width=4.5cm, height=4cm]{./figures/method/5_new.png}};
% % Shortened coarse registration arrow
% \draw[->, >=latex, thick, draw=black] (4.5,5.5) -- (6,5.5);  % Made this arrow shorter
% \node[font=\small, align=center] at (5.2,6) {Coarse \\ Registration};
% \node[img] (img6) at (8.5,5.5) {\includegraphics[width=5cm, height=3cm]{./figures/method/7.png}};
% % Shortened fine registration arrow
% \node[img] (img7) at (14.5,5.5) {\includegraphics[width=6cm, height=4cm]{./figures/method/8_updated2.png}};
% \draw[->, >=latex, thick, draw=black] (11.5,5.5) -- (13,5.5);  % Made this arrow shorter
% \node[font=\small, align=center] at (12.2,6) {Fine \\ Registration};

% % \node[font=\small] at (13.5,7.7) {Results};

% % Labels for the paths
% \node[font=\small] at (8,13.7) {Train 3DGS};
% \node[font=\small] at (8,10.3) {Train 3DGS};
% \end{tikzpicture}
% \caption{\textcolor{red}{Roy: "Unfinished"}}
% \label{fig:method}
% \end{figure*}



Our algorithm iteratively performs two main steps:

\paragraph{Feature-based Correspondence Search} In each iteration \(k\), we establish correspondences based on both feature similarity and spatial proximity. For each point \(\bp_i\), we define its transformed version from the previous iteration:
\begin{align}
    \bp_i^{k-1} = \Tcal^{(k-1)}(\bp_i^{(k-2)}),
\end{align}
where \(\bp_i\) is the initial point and \(\Tcal^{(k-1)}\) is the estimated transformation from the previous iteration.

Next, we identify the feature-compatible subset in \(\Qcal\):
\begin{align}
\Qcal_i = \{\bq_j \in \Qcal \mid \|\boldf_i - \boldf_j\| \leq \tau\}
\end{align}
where \(\tau\) is a feature similarity threshold. Within this subset, we determine the spatially closest point to \(\bp_i^{k-1}\):
\begin{align}
\bq_i^{k} = \underset{\bq \in \Qcal_i}{\text{arg min}} \|\bp_i^{k-1} - \bq\|^2.
\end{align}

\paragraph{Transformation Optimization} Given the correspondences \(\{(\bp_i, \bq_i^{k})\}\), we solve for the optimal transformation parameters by minimizing:
\begin{align}
\Lcal_{\mathrm{Coarse}}^{(k)} &= \sum_{i} \|\Tcal^{(k)}(\bp_i^{k-1}) - \bq_i^{k}\|^2  \notag \\
&= \sum_{i} \|s \bR (\bp_i^{k-1}) + \bt - \bq_i^{k}\|^2.
\end{align}

The optimization follows Horn's method \cite{horn1988closed} for the absolute orientation problem, which provides a closed-form solution for similarity transformations. This generalizes the standard ICP algorithm, which is a special case where \(s = 1\). The solution involves:

\begin{enumerate}
    \item Computing the centroids \(\bar{\bp}^k = \frac{1}{N}\sum_i \bp_i^{k-1}\) and \(\bar{\bq}^k = \frac{1}{N}\sum_i \bq_i^{k}\).
    \item Centering the points \(\bp_i'^k = \bp_i^{k-1} -  \bar{\bp}^k\) and \(\bq_i'^k = \bq_i^{k} - \bar{\bq}^k\).
    \item Computing the optimal scale:
    \begin{align}
    s^k = \sqrt{\frac{\sum_i \|\bq_i'^k\|^2}{\sum_i \|\bp_i'^k\|^2}}.
    \end{align}
    \item Solving for rotation using SVD of the correlation matrix:
    \begin{align}
    \bR^k = \bV^k {\bU^k}^T, \text{ where } \bU^k\bS^k{\bV^k}^T = \sum_i \bq_i'^k {\bp_i'^k}^T.
    \end{align}
    \item Computing translation:
    \begin{align}
    \bt^k = \bar{\bq}^k - s^k\bR^k\bar{\bp}^k.
    \end{align}
\end{enumerate}

The updated transformation is then applied to the points:
\begin{align}
    \bp_i^k = \Tcal^{(k)}(\bp_i^{k-1}) = s^k \bR^k (\bp_i^{k-1}) + \bt^k.
\end{align}

The algorithm iterates between correspondence search and transformation optimization until convergence, defined by either a maximum iteration count or when the change in transformation parameters falls below a threshold \(\epsilon\).


\subsection{Fine Registration: Multi-view Semantic Features Consistency Reprojection Error}


After the coarse alignment using modified ICP, we implement a fine alignment step leveraging multi-view feature map rendering and feature-based loss optimization. This step fundamentally differs from our initial feature learning phase in how gradients flow through the 3D Gaussian representation.

During the initial training of our 3D Gaussian model, the feature vectors were learned concurrently with other Gaussian properties (means, covariances, opacities, and spherical harmonics), but their gradients were isolated. We train these features using the masked feature maps \(F_k^{\text{masked}}\), ensuring that the feature learning process did not influence the geometric properties of the scene. This isolation preserves the spatial integrity of the 3D representation learned directly from the masked images \(I_k^{\text{masked}}\).

In contrast, during our fine alignment optimization, we strategically employ these learned features to guide the geometric transformation. While keeping the Gaussian attributes frozen, we allow gradients from our feature-based loss to propagate through the entire 3D structure, enabling precise optimization of the similarity transformation for different objects with similar geometric semantic meaning. For the target model and the source aligned model (transformed by the coarse registration), we render \( K \) different feature maps from varying viewpoints, denoted as \( F_k^{\text{rend},(1)} \) and \( F_k^{\text{rend},(2)} \) for the \( k \)-th view of models 1 and 2, respectively.

The alignment is refined by minimizing the Mean Squared Error (MSE) loss between the rendered feature maps:

\begin{align}
\Lcal_{MSE} = \frac{1}{K} \sum_{k=1}^{K} \| F_k^{\text{rend},(1)} - F_k^{\text{rend},(2)} \|^2
\end{align}

The key distinction lies in how we apply the similarity transformation to the 3D Gaussians. For each Gaussian, we transform its geometric attributes according to:

\begin{align}
\begin{aligned}
\bp_i' &= s \bR \bp_i + \bt \\
\bSigma_i' &= s \bR \bSigma_i \bR^T
\end{aligned}
\end{align}

where \(\bp_i'\) and \(\bSigma_i'\) represent the transformed mean and covariance respectively. By allowing the features' gradients to flow through these geometric transformations while keeping the original Gaussian attributes frozen, we can optimize the similarity transformation parameters \(s\), \(R\), and \(t\) with high precision. This approach leverages the semantic information captured in our features to guide the geometric alignment while maintaining the structural integrity of each model's representation.

In scenarios where preserving the original scale of the source model is desired, we still utilize the similarity transformation during optimization, as it facilitates finding the optimal rotation and translation parameters robustly utilizing the scale parameter. After completing the alignment, we can restore the original scale by applying an inverse scaling factor of \(1/s\) to the transformed model, where \(s\) is the scale parameter learned during optimization. This approach leverages the flexibility of scale adjustment during the optimization process, enabling better alignment between feature maps of objects that share similar 3D geometry-aware features but may differ in their specific geometric structure. The scale adjustment during optimization helps accommodate these geometric variations in the alignment process, while ultimately preserving the source model's original dimensions in the final result is easy.

For specifically implementation details please refer to the section ... in our supplementary materials.



==> sec/alg_all.tex <==
% \begin{algorithm}[!h]
%     \caption{Gaussian Splatting Alignment}
%     \label{alg:GS3D_registration}
    
%     \KwIn{
%         Feature-augmented 3DGS models \( \Gcal_1, \Gcal_2 \).
%     }
%     \KwOut{
%         Similarity transformation \( T^* = (s, \bR, \bt) \).
%     }
    
%    % \tcp{Coarse Registration via Feature-Guided Absolute Orientation Solver}
%        %\tcp{Coarse Alignment}
%      \( T \gets \) \autoref{alg:coarse_registration} \( (\Gcal_1, \Gcal_2) \)
%     \tcp{Coarse}
%    % \tcp{Fine Registration via Multi-View Feature Consistency}
%   % \tcp{Fine Alignment}
%      \( T^* \gets \)  \autoref{alg:fine_registration} \( (\Gcal_1, \Gcal_2, T) \)
%     \tcp{fine}    
%     \textbf{Return} \( T^* \)
% \end{algorithm}

==> sec/copy_of_3_finalcopy.tex <==
\section{Experiments and Results}\label{Sec:Results}
% \subsection{setup}
\subsection{Registration of Different Models of the same objects}

We evaluated our method using the same dataset evaluation as DregNeRF and GaussReg evaluate within the same categories that can be used in our feature extractor, which contains 15 different objects. 

% \begin{table}[!htb]
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%         Method & RRE (°) ↓ & ATE ↓ \\
%         \midrule
%         REGTR &? & ? \\
%         DReg-NeRF & 10.3742 & 0.0405 \\
%         GaussReg & 18.5967 & 0.0654 \\
%         Ours w/o. fine & 3.1329 &  0.01 \\
%         Ours lightweight & 3.1329 &  0.01 \\
%         Ours & \textbf{0.3585} & \textbf{0.0048} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Quantitative comparison of registration accuracy. RRE: Relative Rotation Error (in degrees), ATE: Absolute Translation Error. Lower values are better (↓).}
%     \label{tab:registration_results}
% \end{table}

\begin{table}[!htb]
    \centering
    \begin{tabular}{lcc}
        \toprule
        Method & RRE (°) ↓ & ATE ↓ \\
        \midrule
        FGR & - & - \\
        REGTR & 52.5356 & 0.3279 \\
        DReg-NeRF & 10.3742 & 0.0405 \\
        GaussReg & 18.5967 & 0.0654 \\
        \midrule
        Ours coarse & 3.1329 & 0.01 \\
        % Ours Efficient w/o. fine & - & - \\
        % Ours Efficient  & - & - \\
          \rowcolor{lightyellow}Ours coarse + fine & \textbf{0.3585} & \textbf{0.0048} \\
        \bottomrule
    \end{tabular}
    \caption{Quantitative comparison of registration accuracy. RRE: Relative Rotation Error (in degrees), ATE: Absolute Translation Error. Lower values are better (↓).}
    \label{tab:single_object_registration_results}
\end{table}


Both GaussReg and DReg-NeRF assume that models share a fixed scale (s = 1). However, in Novel View Synthesis, this assumption is generally incorrect, as Structure-from-Motion (SfM) algorithms assign an arbitrary scale to the initial point cloud due to the lack of depth information in images.

Our primary competitor within the 3D Gaussian Splatting (3DGS) domain, GaussReg, experiences a significant drop in accuracy when the scale is unknown, as it must estimate a full similarity transformation. To address this limitation, GaussReg's evaluation assumes a fixed unit scale (s = 1), reducing the problem to a rigid transformation, a simplification also adopted by DReg-NeRF.

For a fair comparison, we apply the same fixed scale assumption (s = 1) across all evaluated methods, including FGR and REGTR, ensuring that they estimate only a rigid transformation consistent with their original evaluation settings. In contrast, our method effectively determines that the scale is close to 1 without relying on this assumption, demonstrating its robustness under full similarity transformations, which presents a greater challenge.


\subsection{Registration of Different Objects Within Categories}  

We evaluated our method across six distinct object categories from the ShapeNet dataset \TODO{cite shapenet}, which consists of manually aligned 3D models. Within each category, we selected five different objects and generated corresponding images and masks. The quantitative results of our evaluation are summarized in \autoref{tab:method_category_results}.  

To ensure a fair and comprehensive evaluation, we considered all possible object pairs within each category, preventing bias from pairs that might be inherently easier to register. Since each category contains five different objects, we evaluated 10 unique object pairs per category, covering all possible pairwise combinations. Across six categories, this resulted in a total of 60 object pairs.  

For each object pair, we applied a random similarity transformation, including rotation, translation, and scaling, to one of the objects in the pair. We then saved the transformed object as ground truth and evaluated registration accuracy against it. This approach ensures that the evaluation measures how well each method can recover the correct alignment under realistic transformations.  

Given that the objects exhibit diverse geometries and multiple valid solutions exist for both scale and translation, we focused solely on rotation accuracy, measured using Relative Rotation Error (RRE).  

Notably, we did not evaluate against DReg-NeRF, as our primary focus is on the 3D Gaussian Splatting (3DGS) domain. Moreover, we have already demonstrated superior performance over DReg-NeRF in a simpler experimental setup, making further comparisons unnecessary.  


\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1}  
    \setlength{\tabcolsep}{12pt} 
    \begin{tabular}{lcccccc} 
        \toprule
        Method & Airplane & Bus & Boat & Car & Chair & Motorcycle \\
        & RRE (°) ↓ & RRE (°) ↓ & RRE (°) ↓ & RRE (°) ↓ & RRE (°) ↓ & RRE (°) ↓ \\
        \midrule
        FGR & 90.7753 & 94.9839 & 86.5981 & 89.3221 & 91.5310 & 82.0594 \\
        REGTR & 89.9995 & 77.6940 & 90.9799 & 96.9832 & 94.7477 & 86.9677 \\
        GaussReg & 136.3235 & 138.5101 & 126.6419 & 121.3649 & 155.0323 & 120.1386 \\
        \midrule

         Ours w/o. fine & 3.1504 & 4.7420 & 14.7385 & 3.6984 & 14.1742 & \textbf{3.1293} \\
        \rowcolor{lightyellow} Ours & \textbf{2.4870} & \textbf{2.4125} & \textbf{7.7670} & \textbf{1.7106} & \textbf{10.8582} & 4.0475 \\
        \bottomrule
    \end{tabular}
    \vspace{5pt} 
    \caption{\centering Comparison of registration accuracy across different object categories and methods. \\ 
    RRE: Relative Rotation Error (in degrees). Lower values are better (↓).}
    \label{tab:method_category_results}
\end{table*}


\subsection{Registration on Real-World Data}
To evaluate the effectiveness of our method on real-world data, we tested it using the 3D Real Car dataset \TODO{cite 3D Real Car}, with the results summarized in \autoref{tab:3d_real_car_registration_results}. Since ground truth alignments for the models are unavailable, we manually aligned five different 3D Gaussian models to create a small benchmark consisting of five distinct cars, resulting in ten pairwise combinations for evaluation.

Although 3D Real Car proposed a method specifically designed for their car dataset and camera views to bring the initial sparse point cloud from COLMAP into a common coordinate system using PCA on the camera views, this approach was intended to produce aligned 3D models after training. However, in practice, it did not work reliably, especially as ground truth. Therefore, after training, we manually aligned the 3D Gaussian models to ensure an accurate evaluation.

When constructing the 3D Gaussian Splatting (3DGS) models, we used camera views from COLMAP. However, during the manual alignment step after training, we only aligned the 3D models and did not adjust the original camera poses from training. As a result, we evaluate methods that operate purely on point clouds, including our coarse registration, which does not depend on camera views.

Our coarse registration method achieves the best results, demonstrating its effectiveness in point-cloud-based alignment within the 3DGS representation.

\begin{table}[H]
    \centering
    \begin{tabular}{lc}
        \toprule
        Method & RRE (°) ↓ \\
        \midrule
        FGR & 67.7120 \\
        REGTR & 85.8642 \\
        % GaussReg & 118.9435\\
        \rowcolor{lightyellow}Ours Coarse & \textbf{2.3849} \\
        \bottomrule
    \end{tabular}
    \caption{Quantitative comparison of point cloud-based registration. RRE: Relative Rotation Error (in degrees), ATE: Absolute Translation Error. Lower values are better (↓).}
    \label{tab:3d_real_car_registration_results}
\end{table}


\subsection{Implementation Details}

\subsubsection{First Experiment}  
For all variations of our method (Ours w/o. fine, Ours, Ours Efficient, etc.), we set $\tau = 0.01$ for the coarse registration.  

In the efficient version, the coarse registration was performed with only \textbf{3 iterations}, while the fine registration used \textbf{3 to 5 different views} with \textbf{80 iterations}. In contrast, the full version ran the coarse registration until convergence and also used \textbf{80 iterations} for fine registration.  

For fine registration, we applied a \textbf{learning rate of 0.1} to optimize all similarity transformation parameters.  

\subsubsection{Second Experiment}  
For the coarse registration, we set $\tau = 0.01$ with a maximum of \textbf{6 iterations} or until convergence. During fine registration, we selected every \textbf{5th frame} for refinement.  

A \textbf{learning rate of 0.01} was used for optimizing the similarity transformation parameters.


\subsubsection{Third Experiment}  
We evaluate the performance of the real objects using our coarse registration to demonstrate the power of our method compared to the other methods. We set $\tau = 0.01$ with a maximum of \textbf{3 iterations} until convergence.


\subsection{Ablation}  
We experimented with different versions of DINO features. Although DINOv2 provides a higher feature dimension compared to the feature extractor we used, it lacks geometric information, leading to "flipped" solutions—rotations of up to 180 degrees in the opposite direction.  

A similar issue arose with the Telling From Left to Right method. Ambiguity occurred when viewing objects from opposite directions, as the left side in one view corresponded to the right side in another. This resulted in two equally valid solutions, one of which was flipped relative to the ground truth.

For the coarse registration, we tried with different $\tau$ values, but we found that 0.01 is best for all datasets.


==> sec/table_IO.tex <==
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1}
    \setlength{\tabcolsep}{5pt} % Adjust column spacing
    \begin{tabular}{|p{4.5cm}|p{5.5cm}|p{5.5cm}|}
        \hline
        \textbf{Step} & \textbf{Input} & \textbf{Output} \\ \hline
        Building two independent feature-enhanced 3DGS models & 
        2 sets of images \( \{I_i\} \)
        and \( \{J_j\} \), along with 
        estimated camera poses (one per image).
        The sets are not directly related
        to each other, and can also have different numbers of images. & 
        3DGS models \( \Gcal_1, \Gcal_2 \), augmented with with viewpoint-guided spherical features. \\ \hline
        Coarse Registration via a Feature-Guided Absolute Orientation Solver & 
          \( \Gcal_1, \Gcal_2 \), Feature correspondences based on geometric position and feature similarity & 
        Initial similarity transformation \( T=(s, \bR, \bt) \) between
        (the fixed)  \( \Gcal_1\) and  \(\Gcal_2 \).       
      \\ \hline
        Fine Registration via Multi-View Feature Consistency & 
       \( \Gcal_1, \Gcal_2 \) , Initial similarity transformation \( T=(s, \bR, \bt) \)  & 
       Final similarity transformation \( T^*=(s, \bR, \bt) \) between
        (the fixed)  \( \Gcal_1\) and  \(\Gcal_2 \). 
        \\ \hline
    \end{tabular}
    \caption{Overview of the three main steps in our registration pipeline. The 3D Gaussian models remain fixed after their initial construction.}
    \label{Table:MethodOverview}
\end{table*}


==> sec/table_real_ablation.tex <==
\begin{table*}[h]
    \centering
    \caption{Ablation study of our method across different object categories. We analyze the impact of different settings for the coarse and fine stages. Lower values are better ($\downarrow$).}
    \setlength{\tabcolsep}{3pt} % Reduce column spacing
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Configuration} & \textbf{Airplane} & \textbf{Bus} & \textbf{Boat} & \textbf{Car} & \textbf{Chair} & \textbf{Motorcycle} \\
        & RRE (°) $\downarrow$ & RRE (°) $\downarrow$ & RRE (°) $\downarrow$ & RRE (°) $\downarrow$ & RRE (°) $\downarrow$ & RRE (°) $\downarrow$ \\
        \midrule
        GSA (only coarse) - 1 iteration & 91.04 & 86.79 & 83.10 & 95.52 & 84.42 & 82.52 \\
        GSA (only coarse) - 3 iterations & 3.05 &  4.30 & \textbf{25.17} & 3.27 & 14.54 & \textbf{2.81} \\
        GSA (only coarse) - Until convergence & \textbf{2.97} & \textbf{4.06} & 30.21 & \textbf{3.26} & \textbf{10.50} & 2.89 \\
        \midrule
       GSA (coarse 3 iterations  + fine) - 3 (similar) views &  4.23 & 4.56 & 29.10 & 5.15 & 11.54 & 6.05 \\
        GSA (coarse 3 iterations + fine) - 3 (diverse) views & 2.72 & 3.02 & \textbf{22.68} & \textbf{1.88} & 10.26 & 3.94 \\
        GSA (coarse 3 iterations  + fine) - 30 views & \textbf{2.41} & \textbf{2.50} & 22.90 & 1.90 & \textbf{5.97} & \textbf{4.44} \\
        \bottomrule
    \end{tabular}
    \label{tab:ours_ablation}

\end{table*}


==> sec_orig_cvpr/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec_orig_cvpr/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec_orig_cvpr/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec_orig_cvpr/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
